Dual-Perspective Knowledge Enrichment for Semi-Supervised 3D Object Detection

Semi-supervised 3D object detection is a promising yet under-explored direction to reduce data annotation costs, especially for cluttered indoor scenes. A few prior works, such as SESS and 3DIoUMatch, attempt to solve this task by utilizing a teacher model to generate pseudo-labels for unlabeled samples. However, the availability of unlabeled samples in the 3D domain is relatively limited compared to its 2D counterpart due to the greater effort required to collect 3D data. Moreover, the loose consistency regularization in SESS and restricted pseudo-label selection strategy in 3DIoUMatch lead to either low-quality supervision or a limited amount of pseudo labels. To address these issues, we present a novel Dual-Perspective Knowledge Enrichment approach named DPKE for semi-supervised 3D object detection. Our DPKE enriches the knowledge of limited training data, particularly unlabeled data, from two perspectives: data-perspective and feature-perspective. Specifically, from the data-perspective, we propose a class-probabilistic data augmentation method that augments the input data with additional instances based on the varying distribution of class probabilities. Our DPKE achieves feature-perspective knowledge enrichment by designing a geometry-aware feature matching method that regularizes feature-level similarity between object proposals from the student and teacher models. Extensive experiments on the two benchmark datasets demonstrate that our DPKE achieves superior performance over existing state-of-the-art approaches under various label ratio conditions. The source code will be made available to the public.

==> define.tex <==

\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}

\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}

\newcommand{\wrt}{\textit{w.r.t.}}
\newcommand{\eg}{\textit{e.g.}}
\newcommand{\ie}{\textit{i.e.}}
\newcommand{\etal}{\textit{et al.}}

\newcommand{\fprograd}{\hat{f}_{\text{prograd}}}
\newcommand{\fp}{\hat{f}_{\text{p}}}
\newcommand{\fce}{\hat{f}_{\text{ce}}}
\newcommand{\fstu}{{f}_{\text{stu}}}
\newcommand{\ftea}{{f}_{\text{tea}}}
\newcommand{\gprograd}{\bm{G}_\text{prograd}}
\newcommand{\gce}{\bm{G}_\text{ce}}
\newcommand{\gkl}{\bm{G}_\text{kl}}
\newcommand{\gperp}{\bm{G}_{\perp}}
\newcommand{\Dq}{\mathcal{D}_q}
\definecolor{tabhighlight}{HTML}{e5e5e5}

\newcommand{\tableCellHeight}{1}
\newcommand{\tabstyle}[1]{
  \setlength{\tabcolsep}{#1}
  \renewcommand{\arraystretch}{\tableCellHeight}
  \centering
  \small
}

\newcommand{\ours}{App }
\newcommand{\mapa}{\begin{tabular}[c]{@{}c@{}}mAP\\ @0.25\end{tabular}}
\newcommand{\mapb}{\begin{tabular}[c]{@{}c@{}}mAP\\ @0.5\end{tabular}}

==> images/Fig1_old.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}[t]{.65\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/figure1.pdf}
        \caption*{(a)}
    \end{minipage}\quad
    \begin{minipage}[t]{.27\linewidth}
        \centering
        % \vspace{0.1cm} % 向下移动 1cm
        \includegraphics[width=\linewidth]{images/fig1b.pdf}
        \caption*{(b)}
    \end{minipage}
    \caption{(a) Visualization of 3D indoor (ScanNet \cite{dai2017scannet}), 3D outdoor (KITTI \cite{kitti}), 2D (PASCAL VOC \cite{everingham2010pascal}) datasets. (b) The statistics for each dataset. The orange bars represent the number of samples in the corresponding dataset, while the blue bars represent the number of objects per sample.}
    \label{fig:Fig1}
\end{figure*}

==> images/Fig2.tex <==
\setlength\intextsep{0pt}
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{images/figure1b.pdf}
    \caption{Object number per scene/image, and the dataset scale.}
    \label{fig:Fig2}
\end{wrapfigure}

==> images/failurecase.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\textwidth]{images/failurecase.pdf}
\caption{Failure cases analysis. We evaluate the distribution of samples that are mis-classified by \texttt{ProGrad} models but correctly classified by CoOp models on (a) EuroSAT~\cite{eurosat} (b) Oxford Flowers~\cite{flowers102} and UCF101~\cite{ucf101} datasets.}
\label{fig:failurecase}
\end{figure}

==> tables/augmentation_change.tex <==
\begin{table}[t]
\caption{Evaluation on robustness to distribution shift.  The context length $M$ is 16 for all prompt-based methods and the prompts are trained with 4 shots. \textbf{Best} and \underline{\textbf{second best}} results are marked.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|ccccccccccc|}
\hline
Object & cab & bed & chair & sofa & table & door & wind & bkshf & pic & mAP \\
AP change & 0.026 & 0.012 & 0.024 & 0.037 & 0.016 & 0.075 & 0.021 & 0.060 & -0.001 & 0.030 \\ \hline
Object & cntr & desk & curt & fridg & showr & toil & sink & bath & garbagebin & mAP \\ 
AP change & 0.011 & 0.029 & 0.075 & 0.041 & 0.014 & 0.022 & 0.045 & -0.026 & 0.054 & 0.030 \\
\hline
\end{tabular}
}
\label{tab:aug_category}
\end{table}
